Thermal Effects for Quark and Gluon Distributions in Heavy-Ion Collisions

In-medium effects for distributions of quarks and gluons in central A+A collisions are considered. We suggest a duality principle, which means similarity of thermal spectra of hadrons produced in heavy-ion collisions and inclusive spectra which can be obtained within the dynamic quantum scattering theory. Within the suggested approach we show that the mean square of the transverse momentum for these partons grows and then saturates when the initial energy increases. It leads to the energy dependence of hadron transverse mass spectra which is similar to that observed in heavy ion collisions.

==> macros.tex <==

  \def\bSfVer#1{\begin{Slide*}{#1}\begin{figure}\centering}
  \def\eSfVer{\end{figure}\end{Slide*}}
  \def\bSfHor#1{\begin{Slide}{#1}\begin{figure}\centering}
  \def\eSfHor{\end{figure}\end{Slide}}
  \def\bStVer#1{\begin{Slide*}{#1}\begin{table}\centering}
  \def\eStVer{\end{table}\end{Slide*}}
  \def\bStHor#1{\begin{Slide}{#1}\begin{table}}
  \def\eStHor{\end{table}\end{Slide}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Define short aliases for colours                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \def\Colortext#1#2{{#1}{#2}\black{}}
%    
  \def\Rtext#1{\red{#1}\black{}}
  \def\Gtext#1{\green{#1}\black{}}
  \def\Btext#1{\blue{#1}\black{}}
  \def\Ctext#1{\cyan{#1}\black{}}
  \def\Mtext#1{\magenta{#1}\black{}}
  \def\Ytext#1{\yellow{#1}\black{}}
  \def\Ptext#1{\paleyellow{#1}\black{}}
  \def\Atext#1{\amber{#1}\black{}}
%
  \def\dRtext#1{\darkred{#1}\black{}}
  \def\dGtext#1{\darkgreen{#1}\black{}}
  \def\dBtext#1{\darkblue{#1}\black{}}
  \def\dCtext#1{\darkcyan{#1}\black{}}
  \def\dMtext#1{\darkmagenta{#1}\black{}}
  \def\dYtext#1{\darkyellow{#1}\black{}}
  \def\dAtext#1{\darkamber{#1}\black{}}
%
  \def\lRtext#1{\lightred{#1}\black{}}
  \def\lGtext#1{\lightgreen{#1}\black{}}
  \def\lBtext#1{\lightblue{#1}\black{}}
  \def\lCtext#1{\lightcyan{#1}\black{}}
  \def\lMtext#1{\lightmagenta{#1}\black{}}
  \def\lYtext#1{\lightyellow{#1}\black{}}

%-------------------------------------------------------------------%
%  Redefine aliases for sectionung and references to sections       % 
%-------------------------------------------------------------------%

% \def\Chapter#1#2%
%    {\protect\dRtext{\chapter[\dRtext{#1}]{#1}\label{#2}}}
  \def\Chapter#1#2%
     {\protect\dRtext{\section[\dRtext{#1}]{#1}\label{#2}}}
  \def\ChapRef#1%
     {\;\Rtext{\bf{\ref{#1}}}\;}
% ...................................................................
% \def\Section0#1{\protect\dAtext{\section*{#1}}}
  \def\Section0#1{\protect\dAtext{\subsection*{#1}}}
% ...................................................................
% \def\Section#1#2{\protect\dAtext{\section{#1}\label{#2}}}
  \def\Section#1#2{\protect\dAtext{\subsection{#1}\label{#2}}}
  \def\SectRef#1{\;\dAtext{\bf{\ref{#1}}}\;}
% ...................................................................
% \def\SubSection#1#2{\protect\Atext{\subsection{#1}\label{#2}}}
  \def\SubSection#1#2{\protect\Atext{\subsubsection{#1}\label{#2}}}
  \def\SubSectRef#1{\;\Atext{\bf{\ref{#1}}}\;}
% ...................................................................
% \def\SubSubSection#1#2%
%    {\protect\dCtext{\subsubsection{#1}\label{#2}}}
  \def\SubSubSection#1{\protect\dCtext{\sl{#1}}}
% \def\SubSubSectRef#1{\;\dCtext{\bf{\ref{#1}}}\;}
% ...................................................................
% \def\NOTE#1{\protect\dYtext{\bf\underline{#1}}}
  \def\NOTE#1{\protect\dYtext{\bf\underline{#1}}\vskip 1mm}
% \def\NOTE#1{\vskip 1mm \protect\dYtext{\bf\underline{#1}}%
%     \vskip 1mm}

% ...................................................................
  \def\PROBLEM {\protect\dAtext{\sl\underline{Problem}: }}
  \def\PROBLEMS{\protect\dAtext{\sl\underline{Problems}:}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Define short aliases for formulas                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newcommand{\PS}{\mathfrak{M}_{\mathbf{r},\mathbf{p}}}
% \newcommand{\PS}{\mathfrak{M}_{\mathbf{r}}\otimes%
%                                \mathfrak{M}_{\mathbf{p}}}

  \newcommand{\PS}{\mathbb{R}_{\mathbf{r}}\otimes%
                               \mathbb{R}_{\mathbf{p}}}
% \newcommand{\tg}{\mathrm{tg}\,}
% \newcommand{\tg}{\mathop\mathrm{tg}\nolimits}
  \def\tg{\mathop{\rm tg}\nolimits}
  \def\cotg{\mathop{\rm cotg}\nolimits}
  \def\arctg{\mathop{\rm arctg\nolimits}}
  \newcommand{\nablan}{\nabla_{\!\mathbf{n}}\,}
  \newcommand{\nablank}{\nabla_{\!\mathbf{n}_k}\,}
  \newcommand{\nablanmod}{\nabla_{\!\mathbf{n}'}\,}
  \newcommand{\nequiv}{\equiv\!\!\!\!\!/\;\;}
  \newcommand{\thetafunc}{\mathop\theta}
%
  \newcommand{\pL}{p\strut_{{}^\|}}
  \newcommand{\pLp}{p\strut_{{}^\|}^{\prime}}
  \newcommand{\pLt}{\widetilde{p}\strut_{{}^\|}}
  \newcommand{\pLpt}{\widetilde{p}\strut_{{}^\|}^{\;\prime}}
  \newcommand{\pT  }{p\strut_\bot}
  \newcommand{\pTp }{p\strut_\bot^{\prime}}
  \newcommand{\pTt }{\widetilde{p}\strut_\bot}
  \newcommand{\pTpt}{\widetilde{p}\strut_\bot ^{\;\prime}}
% 
  \newcommand{\vL}{v\strut_{{}^\|}}
  \newcommand{\vLp}{v\strut_{{}^\|}^{\prime}}
  \newcommand{\vLt}{\widetilde{v}\strut_{{}^\|}}
  \newcommand{\vLpt}{\widetilde{v}\strut_{{}^\|}^{\;\prime}}
  \newcommand{\vT  }{v\strut_\bot}
  \newcommand{\vTp }{v\strut_\bot^{\prime}}
  \newcommand{\vTt }{\widetilde{v}\strut_\bot}
  \newcommand{\vTpt}{\widetilde{v}\strut_\bot ^{\;\prime}}
%
  \def\L#1{{#1}\strut_{{}^\|}}
  \def\Lp#1{{#1}\strut_{{}^\|}^{\prime}}
  \def\Lt#1{\widetilde{#1}\strut_{{}^\|}}
  \def\Lpt#1{\widetilde{#1}\strut_{{}^\|}^{\;\prime}}
  \def\T#1{{#1}\strut_\bot}
  \def\Tp#1{{#1}\strut_\bot^{\prime}}
  \def\Tt#1{\widetilde{#1}\strut_\bot}
  \def\Tpt#1{\widetilde{#1}\strut_\bot^{\;\prime}}
%
  \newcommand{\Pol}{\mathcal{P}}
%
  \newcommand{\dif}{d}         % \newcommand{\dif}{\mathrm{d}}
  \newcommand{\diff}{d^{\,2}}  % \newcommand{\diff}{\mathrm{d}^2}
  \newcommand{\difff}{d^{\,3}} % \newcommand{\difff}{\mathrm{d}^3}
  \newcommand{\sign}{\text{sign}}
  \newcommand{\eV }{\text{eV}}
  \newcommand{\keV}{\text{keV}}
  \newcommand{\MeV}{\text{MeV}}
%  \newcommand{\GeV}{\text{GeV}}
  \newcommand{\TeV}{\text{TeV}}
  \newcommand{\PeV}{\text{PeV}}
  \newcommand{\EeV}{\text{EeV}}
  \newcommand{\ZeV}{\text{ZeV}}
%  \newcommand{\cm}{\text{cm}}
  \newcommand{\km}{\text{km}}
  \newcommand{\s}{\text{s}}

  \newcommand{\mwe}{\text{m.\,w.\,e.}}
  \newcommand{\mb}{\text{mb}}
  \newcommand{\mub}{\mu\text{b}}
  \newcommand{\g}{\text{g}}
  \newcommand{\hg}{\text{hg}}
  \newcommand{\vs}{{\em vs}\;}
  \newcommand{\ktyr}{kt$\cdot$yr}
  \newcommand{\nuf}{|\nu\rangle\strut_{\text{f}}}
  \def\nuft#1{|\nu(#1)\rangle\strut_{\text{f}}}
  \newcommand{\num}{|\nu\rangle\strut_{\text{m}}}
  \def\numt#1{|\nu(#1)\rangle\strut_{\text{m}}}
  \newcommand{\FrontNote}{\footnotetext{\hspace{-5mm}\dBtext%
  {\scriptsize V.\,A.\,Naumov, Dubna, September, 2004}}}

 \def\NOE    {{\em    N\raise.5ex\hbox{O \kern-0.47em}E\kern.4em}}
 \def\NoE    {        N\raise.5ex\hbox{O \kern-0.47em}E\kern.4em }
 \def\ICANOE {{\em ICAN\raise.5ex\hbox{O \kern-0.47em}E\kern.4em}}
 \def\ICANoE {     ICAN\raise.5ex\hbox{O \kern-0.47em}E\kern.4em }

% \newcommand{\eq}[1]{{\rm (\ref{#1})}}
% \newcommand{\eq}[1]{~{\rm (\ref{eq:#1})}}
% \newcommand{\sys}[1]{~{\rm (\ref{sys:#1})}}
% \newcommand{\scatola}[1]{\Blue\fbox{$\displaystyle #1$}\Black}

\def\rs{\fontencoding{U}\fontfamily{pzd}\selectfont\Red{\symbol{51}}}
\def\gs{\fontencoding{U}\fontfamily{pzd}\selectfont\darkgreen{\symbol{51}}}
\def\ps{\phantom{\rs}}
\def\point{{\black{.}}}
\def\coma{{\black{,}}}
\def\pointcoma{{\black{;}}}

%-------------------------------------------------------------------%

% \def\fa{$\black{{}^{\tiny *)}}$\;}
% \def\fb{$\black{{}^{**)}}$\;}
% \def\fc{$\black{{}^{***)}}$\;}

  \def\fa{$\dMtext{{}^{a}}$\;}   \def\fab{$\dMtext{{}^{a,b}}$\;}
  \def\fb{$\dMtext{{}^{b}}$\;}   \def\fac{$\dMtext{{}^{a,c}}$\;}
  \def\fc{$\dMtext{{}^{c}}$\;}   \def\fbc{$\dMtext{{}^{b,c}}$\;}

  \def\name#1{\begin{center}{ #1 }\end{center}}
  \def\SPIRES#1{\\{}\href{#1}}
  \def\TabEq{&\hspace{-3mm}$=$&\hspace{-3mm}}
  \def\therefore{\quad\Btext{\Rightarrow}\quad}
  \def\Therefore{\[\dRtext{\Downarrow}\]}

  \def\From#1{\scriptsize{\dCtext{[#1]}}}

  \def\sframe#1{\vspace{0.8mm}\Green\bc%
      \fbox{\parbox{16cm}{{\small{#1}}}}\ec\vspace{0.8mm}\Black}
  \def\Bnframe#1{\vspace{-3mm}\Btext{\bc%
      \fbox{\parbox{85mm}{{#1}}}\ec}\vspace{3mm}}

  \def\tick{\ding{52}}

  \def\cbox{\centering\psframebox[fillstyle=solid,%
       fillcolor=paleyellow,framearc=0.2,framesep=2.0mm]}
  \def\rbox{\centering\psframebox[fillstyle=solid,%
       fillcolor=paleyellow,framearc=0.0,framesep=0.0mm]}
  \def\lbox{\centering\psframebox[fillstyle=solid,%
       fillcolor=lightmagenta,framearc=0.0,framesep=1.0mm]}
  \def\BOX#1{\centering\psframebox[fillstyle=solid,%
       fillcolor=lightcyan,framearc=0.0,framesep=#1]}

  \def\BeginDelim{\Blue\name%
     {*****************************************************}}
  \def\EndDelim{\name%
     {*****************************************************}\Black}

  \def\confbox{\centering\psframebox[fillstyle=solid,%
       fillcolor=lightgray,framearc=0.0,framesep=0.5mm]}
  \def\conf{{\scriptsize\confbox{\darkblue Seminar BLTP}}}


% \def\xq{\xi_q}                        % \def\xq{\xi}
% \def\xa{\xi_\overline{q}}             % \def\xa{\xi}  
% \def\xc{\xi_{q,\overline{q}}}         % \def\xc{\xi}  

  \newcommand{\bc}{\begin{center}}
  \newcommand{\ec}{\end{center}}

  \renewcommand{\labelitemi  }{\ding{70}}
  \renewcommand{\labelitemii }{{\small\ding{108}}}
  \renewcommand{\labelitemiii}{$\m@th\rhd$}
  \renewcommand{\labelitemiv }{\rule[1mm]{2.5mm}{0.7mm}}

  \def\Footnote#1{\footnote{#1}}


%-------------------------------------------------------------------%
% Notation for ERS model section:                                   %
%-------------------------------------------------------------------%

 \def\Q{\mathcal{Q}}

 \def\sp#1{\left(#1\right)}
 \def\ml{m}                  % \def\ml{m_\ell}
 \def\Q{{\mathcal Q}}
 \def\lpm{\eta\strut_{\pm\lambda}\eta\strut_{\pm\lambda'}}
 \def\lmp{\eta\strut_{\mp\lambda}\eta\strut_{\mp\lambda'}}
 \def\llp{\eta\strut_{ \lambda\lambda'}}
 \def\llm{\eta\strut_{-\lambda\lambda'}}

 \def\a{\dRtext{****}}
 \def\b{\dGtext{***}}
 \def\c{\dBtext{**}}
 \def\d{*}
%-------------------------------------------------------------------%

\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\cs}[1]{\langle\sigma_{#1}\rangle}
\newcommand{\cse}[1]{\cs{#1}\;\varepsilon^i_{#1}}

